Revisiting Call-by-value B\"ohm trees in light of their Taylor expansion

The call-by-value lambda calculus can be endowed with permutation rules, arising from linear logic proof-nets, having the advantage of unblocking some redexes that otherwise get stuck during the reduction. We show that such an extension allows to define a satisfying notion of B\"ohm(-like) tree and a theory of program approximation in the call-by-value setting. We prove that all lambda terms having the same B\"ohm tree are observationally equivalent, and characterize those B\"ohm-like trees arising as actual B\"ohm trees of lambda terms. We also compare this approach with Ehrhard's theory of program approximation based on the Taylor expansion of lambda terms, translating each lambda term into a possibly infinite set of so-called resource terms. We provide sufficient and necessary conditions for a set of resource terms in order to be the Taylor expansion of a lambda term. Finally, we show that the normal form of the Taylor expansion of a lambda term can be computed by performing a normalized Taylor expansion of its B\"ohm tree. From this it follows that two lambda terms have the same B\"ohm tree if and only if the normal forms of their Taylor expansions coincide.

==> include/Taylor.tex <==
% !TEX root = ../KMP18.tex



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../KMP19.tex"
%%% End:

